Parameter Estimation with Dense and Convolutional Neural Networks Applied to the FitzHugh-Nagumo ODE

Machine learning algorithms have been successfully used to approximate nonlinear maps under weak assumptions on the structure and properties of the maps. We present deep neural networks using dense and convolutional layers to solve an inverse problem, where we seek to estimate parameters of a FitzHugh-Nagumo model, which consists of a nonlinear system of ordinary differential equations (ODEs). We employ the neural networks to approximate reconstruction maps for model parameter estimation from observational data, where the data comes from the solution of the ODE and takes the form of a time series representing dynamically spiking membrane potential of a biological neuron. We target this dynamical model because of the computational challenges it poses in an inference setting, namely, having a highly nonlinear and nonconvex data misfit term and permitting only weakly informative priors on parameters. These challenges cause traditional optimization to fail and alternative algorithms to exhibit large computational costs. We quantify the prediction errors of model parameters obtained from the neural networks and investigate the effects of network architectures with and without the presence of noise in observational data. We generalize our framework for neural network-based reconstruction maps to simultaneously estimate ODE parameters and parameters of autocorrelated observational noise. Our results demonstrate that deep neural networks have the potential to estimate parameters in dynamical models and stochastic processes, and they are capable of predicting parameters accurately for the FitzHugh-Nagumo model.

==> setup_colors_jr.tex <==
% Set of colors
%
% Author: Johann Rudi

% Main colors for text highlighting
\makeatletter%
\@ifclassloaded{beamer}%
  {}% if beamer document class
  {
    \definecolor{jr@darkred}{RGB}{153,0,0}
    \definecolor{jr@medred}{RGB}{204,51,51}
    \definecolor{jr@darkgreen}{RGB}{0,102,0}
    \definecolor{jr@lightgreen}{RGB}{233,255,233}
    \definecolor{jr@darkcyan}{RGB}{51,102,102}
    \definecolor{jr@lightcyan}{RGB}{233,255,255}
    \definecolor{jr@darkgray}{RGB}{51,51,51}
    \definecolor{jr@medgray}{RGB}{102,102,102}
    \definecolor{jr@lightgray}{RGB}{229,229,229}
  }% otherwise
\makeatother%

% Qualitative colorset `9-class Set1` (print friendly, LCD friendly)
% [colorbrewer2.org]
\definecolor{jr@red}{RGB}{228,26,28}
\definecolor{jr@blue}{RGB}{55,126,184}
\definecolor{jr@green}{RGB}{77,175,74}
\definecolor{jr@purple}{RGB}{152,78,163}
\definecolor{jr@orange}{RGB}{255,127,0}
\definecolor{jr@yellow}{RGB}{255,255,51}
\definecolor{jr@brown}{RGB}{166,86,40}
\definecolor{jr@pink}{RGB}{247,129,191}
\definecolor{jr@gray}{RGB}{153,153,153}

% Diverging colorset `6-class RdBu` (print friendly, colorblind save)
% [colorbrewer2.org]
\definecolor{jr@div-darkred}{RGB}{178,24,43}
\definecolor{jr@div-medred}{RGB}{239,138,98}
\definecolor{jr@div-lightred}{RGB}{253,219,199}
\definecolor{jr@div-lightblue}{RGB}{209,229,240}
\definecolor{jr@div-medblue}{RGB}{103,169,207}
\definecolor{jr@div-darkblue}{RGB}{33,102,172}

% Diverging colorset `8-class RdBu` (colorblind save)
% [colorbrewer2.org]
\definecolor{jr@div-red4}{RGB}{178,24,43}
\definecolor{jr@div-red3}{RGB}{214,96,77}
\definecolor{jr@div-red2}{RGB}{244,165,130}
\definecolor{jr@div-red1}{RGB}{253,219,199}
\definecolor{jr@div-blue1}{RGB}{209,229,240}
\definecolor{jr@div-blue2}{RGB}{146,197,222}
\definecolor{jr@div-blue3}{RGB}{67,147,195}
\definecolor{jr@div-blue4}{RGB}{33,102,172}

% Diverging colorset `8-class PRGn` (colorblind save)
% [colorbrewer2.org]
\definecolor{jr@div-purple4}{RGB}{118,42,131}
\definecolor{jr@div-purple3}{RGB}{153,112,171}
\definecolor{jr@div-purple2}{RGB}{194,165,207}
\definecolor{jr@div-purple1}{RGB}{231,212,232}
\definecolor{jr@div-green1}{RGB}{217,240,211}
\definecolor{jr@div-green2}{RGB}{166,219,160}
\definecolor{jr@div-green3}{RGB}{90,174,97}
\definecolor{jr@div-green4}{RGB}{27,120,55}

% Color definitions from ICES
\definecolor{ices@orange}{RGB}{191,87,0}
\definecolor{ices@cyanblue}{RGB}{94,156,174}
\definecolor{ices@lightcyanblue}{RGB}{91,198,232}
\definecolor{ices@darkcyanblue}{RGB}{57,74,88}
\definecolor{ices@verydarkcyanblue}{RGB}{55,66,74}
\definecolor{ices@gray}{RGB}{200,201,199}
\definecolor{ices@green}{RGB}{114,206,155}
\definecolor{ices@yellow}{RGB}{242,169,0}


